Making Secure Software Insecure without Changing Its Code: The Possibilities and Impacts of Attacks on the DevOps Pipeline

Companies are misled into thinking they solve their security issues by using a DevSecOps system. This paper aims to answer the question: Could a DevOps pipeline be misused to transform a securely developed application into an insecure one? To answer the question, we designed a typical DevOps pipeline utilizing Kubernetes (K8s} as a case study environment and analyzed the applicable threats. Then, we developed four attack scenarios against the case study environment: maliciously abusing the user's privilege of deploying containers within the K8s cluster, abusing the Jenkins instance to modify files during the continuous integration, delivery, and deployment systems (CI/CD) build phase, modifying the K8s DNS layer to expose an internal IP to external traffic, and elevating privileges from an account with create, read, update, and delete (CRUD) privileges to root privileges. The attacks answer the research question positively: companies should design and use a secure DevOps pipeline and not expect that using a DevSecOps environment alone is sufficient to deliver secure software.

==> Extras/notes.tex <==
    \begin{procedure}
	 $(n, m, q, A', B', G)\leftarrow f$\\
	  \For{$ i \in \left \{1, . . . , n+q-m \right \}$}
	  {
	  $t \twoheadleftarrow \left \{0,1 \right \}, X^0_i \twoheadleftarrow \left \{0,1\right \}^{k-1}t, X^1_i \twoheadleftarrow \left \{0,1\right \}^{k-1}\bar{t}$

	  }
	  \For{$(g, i, j) \in {n+1, . . . , n+q} \times {0,1} \times {0,1}$}
	  {
	   $a \leftarrow A'(g), b \leftarrow B'(g)$
	  $ A \leftarrow X_a^i, a \leftarrow lsb(A), B \leftarrow X_b^j, b \leftarrow lsb(B)$\\ 
	  $T \leftarrow g\left \| a \right \|b, P\left [ g,a,b \right ] \leftarrow E^T_{A,B}(X_g^{G^{(i,j)}})$
	  }

$ F \leftarrow (n, m, q, A', B', P)$\\
$ e \leftarrow (X^0_1, X^1_1, . . . , X^0_n, X^1_n)$\\
$d \leftarrow (X^0_{n+q-m+1},X^1_{n+q-m+1},...,X^0_{n+q},X^1_{n+q}$

    \Return $(F,e,d)$\\
	\caption{Gb($1^k$,$f$)~\cite{BHR2012}}
	\label{proc:Gb}
\end{procedure}

\begin{lstlisting}[language=C, caption= Structure for garbled circuit object, label=garbledCircuit]

typedef struct {
	int n, m, q, r;
	block* inputLabels, outputLabels;
	GarbledGate* garbledGates;
	GarbledTable* garbledTable;
	Wire* wires;
	int *outputs;
	long id;
	block globalKey;
} GarbledCircuit;
\end{lstlisting}

==> acronym.tex <==


